Full-Duplex Wideband mmWave Integrated Access and Backhaul with Low Resolution ADCs

We consider a wideband integrated access and backhaul system operating in full-duplex mode between the New Radio gNB donor and single user equipment. Due to high power consumption in millimeter wave systems, we use low-resolution analog-to-digital converters (ADCs) in the receivers. Our contributions include (1) hybrid beamformer to maximize sum spectral efficiency of the access and backhaul links by canceling self-interference and maximizing received power; (2) all-digital beamformer and upper bound on sum spectral efficiency; and (3) simulations to compare full vs. half duplex, finite vs. infinite ADC resolution, hybrid vs. all-digital beamforming, and the upper bound in spectral efficiency.

==> performance.tex <==
\section{Performance Analysis}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/hardware.pdf}
    \caption{Basic abstraction of a hybrid combiner.}
    \label{system}
\end{figure}
\subsection{Energy Efficiency}
The energy efficiency, expressed in bits/s/Watt or bits/Joule, is defined as the ratio between the spectral efficiency and the total power consumption. It is expressed as
\begin{equation}
\mathcal{J}(\mathsf{sqinr}) = \frac{\mathcal{I}(\mathsf{sqinr})}{\rho_{\text{Total}}}    
\end{equation}
Where $\rho_{\text{Total}}$ is the total power consumption. For full-digital and hybrid combiners (DC and HC), the total power consumption model for each architecture is defined by
\begin{equation}
\rho^{\text{DC}}_{\text{Total}} =   N_{\text{RX}} \left(\rho_{\text{LNA}} + \rho_{\text{RF}} + 2\rho_{\text{ADC}}  \right) 
\end{equation}
\begin{equation}
\rho^{\text{HC}}_{\text{Total}} = N_{\text{RX}}\left( \rho_{\text{LNA}} + \rho_{\text{SP}} + N_{\text{RF}}\rho_{\text{PS}}  \right) +  N_{\text{RF}} \left( \rho_{\text{RF}} + \rho_{\text{C}} + 2\rho_{\text{ADC}} \right)
\end{equation}
Where $\rho_{\text{RF}}$ is the power consumption per RF chain which is defined by
\begin{equation}
\rho_{\text{RF}} = \rho_{\text{M}} + \rho_{\text{LO}} + \rho_{\text{LPF}} + \rho_{\text{B}\text{B}_{\text{amp}} }    
\end{equation}
\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{Power Consumption of Each Device \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Device & \bfseries Notation & \bfseries Value\\
\hline
Low Noise Amplifier (LNA) \cite{adc36} & $\rho_{\text{LNA}}$ & 39 mW\\
Splitter & $\rho_{\text{SP}}$ & 19.5 mW\\
Combiner \cite{adc36} & $\rho_{\text{C}}$ & 19.5 mW\\
Phase Shifter \cite{adc37,adc38} & $\rho_{\text{PS}}$ & 2 mW\\
Mixer \cite{adc39} & $\rho_{\text{M}}$  & 16.8 mW\\
Local Oscillator \cite{adc27} & $\rho_{\text{LO}}$ & 5 mW\\
Low Pass Filter \cite{adc27} & $\rho_{\text{LPF}}$ & 14 mW\\
Baseband Amplifier \cite{adc27} & $\rho_{\text{B}\text{B}_{\text{amp}} }$ & 5 mW\\
ADC & $\rho_{\text{ADC}}$ & $cB2^b$
\end{tabular}
\end{table}

\begin{table}[H]
\renewcommand{\arraystretch}{1}
\caption{ADC Power Consumption Per Sample Per Level, $c$ \cite{adc}.}
\label{param}
\centering
\begin{tabular}{rll}
\bfseries Scenario & \bfseries Value & \bfseries Generation\\
\hline
LPADC & 5 fJ/step/Hz & Ideal future value\\
IPADC & 65 fJ/step/Hz & Intermediate Power\\
HPADC & 494 fJ/step/Hz & State of the art\\
\end{tabular}
\end{table}

\subsection{Outage Probability}
Once a transmission strategy is specified, the corresponding outage probability for rate $R$ (bits/s/Hz) is then
\begin{equation}
    P_{\textsf{out}}(\mathsf{sqinr}, R) = \mathbb{P}[\mathcal{I}(\mathsf{sqinr})<R ].
\end{equation}
With convenient powerful channel codes, the probability of error when there is no outage is very small and hence the outage probability is an accurate approximation for the actual block error probability. As justified in the literature, modern radio systems such as UMTS and LTE operate at a target error probability. Therefore, the primary performance metric is the maximum rate\footnote[2]{In this work, we define the notion of rate with outage as the average data rate that is correctly received/decoded at the receiver which is equivalent to the throughput. In other standards in the literature, the rate with outage is assimilated with the transmit data rate. The only difference is if we consider rate with outage as the throughput, we account for the probability of bursts (outage) and we multiply by the term (1-$\epsilon$), while for the transmit data rate, the term (1-$\epsilon$) is not accounted anymore.}, at each $\mathsf{sqinr}$, such that this threshold is not overtaken, i.e.,
\begin{equation}
R_\epsilon(\mathsf{sqinr}) = \max_{\zeta}\left\{ \zeta: P_{\textsf{out}}(\mathsf{sqinr}, \zeta) \leq \epsilon \right\}
\end{equation}
where $\epsilon$ is the target.
